Out-of-Distribution Learning with Human Feedback

Out-of-distribution (OOD) learning often relies heavily on statistical approaches or predefined assumptions about OOD data distributions, hindering their efficacy in addressing multifaceted challenges of OOD generalization and OOD detection in real-world deployment environments. This paper presents a novel framework for OOD learning with human feedback, which can provide invaluable insights into the nature of OOD shifts and guide effective model adaptation. Our framework capitalizes on the freely available unlabeled data in the wild that captures the environmental test-time OOD distributions under both covariate and semantic shifts. To harness such data, our key idea is to selectively provide human feedback and label a small number of informative samples from the wild data distribution, which are then used to train a multi-class classifier and an OOD detector. By exploiting human feedback, we enhance the robustness and reliability of machine learning models, equipping them with the capability to handle OOD scenarios with greater precision. We provide theoretical insights on the generalization error bounds to justify our algorithm. Extensive experiments show the superiority of our method, outperforming the current state-of-the-art by a significant margin.

==> chap/learning.tex <==

\section{Learning Framework}

In this section, we delve into the learning pipeline that utilizes wild data, focusing on its application in OOD generalization and detection. These elements are crucial for the effective deployment of machine learning models in real-world scenarios.
A significant challenge in this context is the scarcity of labeled data for scenarios not previously encountered by the model, as well as for training the model to identify OOD samples.
Our active learning-based framework addresses this challenge by enabling the model to efficiently utilize wild data with minimal supervision by focusing on labeling the most informative or uncertain examples. The scarcity of supervised examples in wild data for OOD generalization and detection poses a considerable challenge, yet our learning pipeline, empowered by active learning strategies, offers an effective solution.


\subsection{Learning Pipeline via Active Learning}\label{sec:learning_framework}

\textbf{Learning goal.} Our learning framework aims to select the \textbf{most uncertain or informative} unlabeled data from the wild data and annotate the selected samples of the form of category labels with abstention: $\hat{h}:\mathcal{X} \rightarrow \mathcal{Y} \cup \{ \perp \}$.  Then, (1) building an OOD detector $g_\theta \colon \X \to \{\textsc{in}, \textsc{out} \}$, and (2) training multi-class classifier $h_\theta$ by leveraging data from both $P_\text{in}$ and the most informative data from $P_\text{wild}$ for enhancing OOD generalization accuracy. 
The stopping criteria are to iterate through the active learning cycles of selection, annotation, and refinement until attaining the desired level of performance or exhausting the entire budget allocated for annotations.

In evaluating our model, we are interested in the following measurements:
\begin{align*}
& (1)~\uparrow \text{ID-Acc}(h_\theta):=\mathbb{E}_{(\*x, y) \sim \P_{\mathcal{X}\mathcal{Y}}}(\mathbbm{1}{\{{\widehat{y}(f_\theta(\*x))}=y\}}),\\
&(2)~\uparrow \text{OOD-Acc}(h_\theta):=\mathbb{E}_{(\*x, y) \sim \P_\text{out}^\text{covariate}}(\mathbbm{1}{\{{\widehat{y}(f_\theta(\*x))}=y\}}),\\
&(3)~\downarrow \text{FPR}(g_\theta):=\mathbb{E}_{\*x \sim \P_\text{out}^\text{semantic}}(\mathbbm{1}{\{g_\theta(\*x)=\textsc{in}\}}),
\end{align*}

where $\mathbbm{1}\{\cdot\}$ is the indicator function and the arrows indicate higher/lower is better. ID-Acc, OOD-Acc, and FPR jointly capture the \textbf{(1)} ID generalization, \textbf{(2)} OOD generalization, and \textbf{(3)} OOD detection performance, respectively. In the context of OOD detection, ID samples are considered positive, and FPR means false positive rate. 



\subsection{Three Selection Criteria}\label{learn:selection-criteria}

\textbf{Sample selection procedure.} 
It is expensive to manually label examples for the wild $\mathbb{P}_\text{wild}$ to obtain true labels for training robust multi-class classifiers and identifying the semantic-shifted OOD class. Therefore, the key to active learning for learning with wild data is to design the selection procedure for identifying the most informative samples for labeling to reduce the labeling cost. Such informative samples for OOD generalization and detection are often presented near the decision boundary of the multi-class classifier $h_\theta$ and the decision boundary between the OOD detector $g_\theta$. By leveraging such examples, we can train the multi-class classifier and the OOD detector with far fewer labeled samples.



\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\textwidth]{icml2023/three-sampling.png}
\caption{Illustration of three selection criteria, (1) low likelihood; (2) boundary selection, and (3) mixture of the two. (placeholder) \SL{Very pixelated.}}
\label{fig:select-criteria}
\end{figure*}


Here are the three selection criteria for exploiting wild data specifically designed for OOD generalization and detection:

\begin{itemize}  
\color{red}{\item \textbf{Low likelihood:} These are wild examples that have a low fit to the underline ID distribution (see Figure~\ref{fig:select-criteria} (a)), based on scores $s$ (as detailed in Section~\ref{meth:overview}). These suspected examples lie on the decision boundary of the multi-class classifier. It would be desirable to label these samples for OOD generalization.}

\item \textbf{Boundary selection:} Some examples have the greatest uncertainty between ID distribution and semantic-shifted OOD. By labeling these data, we can learn knowledge about the decision space of ID and semantic OOD samples, thus facilitating OOD detection.
As shown in Figure~\ref{fig:select-criteria} (b), the threshold is determined using ID data $\mathcal{D}_{\text{in}}$ to encompass a substantial proportion (e.g., $95\%$) of in-distribution samples.

\item \textbf{Mixture of the two selection criteria:}
We anticipate that boundary selection is more effective for OOD detection, leveraging data near the decision boundary for a clear distinction between in-distribution and OOD samples. Conversely, low likelihood is preferable for OOD generalization, targeting tail samples with heightened uncertainty. For an optimal balance between detection and generalization, the hybrid approach for mixing the two selection criteria allows us to fine-tune sampling parameters like $N_1$ and $N_2$, enabling us to select samples from both ranges adaptively (see Figure~\ref{fig:select-criteria} (c)).
\end{itemize}






\section{Theoretical Studies}


